Heavy-Meson Spectrum Tests of the Oktay--Kronfeld Action

We present heavy-meson spectrum results obtained using the Oktay--Kronfeld (OK) action on MILC asqtad lattices. The OK action was designed to improve the heavy-quark action of the Fermilab formulation, such that heavy-quark discretization errors are reduced. The OK action includes dimension-6 and -7 operators necessary for tree-level matching to QCD through order $\mathrm{O}(\Lambda^3/m_Q^3)$ for heavy-light mesons and $\mathrm{O}(v^6)$ for quarkonium, or, equivalently, through $\mathrm{O}(a^2)$ with some $\mathrm{O}(a^3)$ terms with Symanzik power counting. To assess the improvement, we extend previous numerical tests with heavy-meson masses by analyzing data generated on a finer ($a \approx 0.12\;$fm) lattice with the correct tadpole factors for the $c_5$ term in the action. We update the analyses of the inconsistency parameter and the hyperfine splittings for the rest and kinetic masses.

==> refs.tex <==
\begin{thebibliography}{99}

%\bibitem{Jang2012:PoS.LAT2012.269}
%Y.-C. Jang and W. Lee,
%\pos{PoS(LATTICE2012)269}
%[{\tt hep-lat/1211.0792}].
%
%\bibitem{swmebk}
%W.~Lee [SWME], these proceedings.
%
%\bibitem{JackVcb}
%S.~Qiu, C.~DeTar, A.S.~Kronfeld {\it et al.} [FNAL/MILC], these proceedings.
%
\bibitem{Wlee}
J.~A.~Bailey {\it et al}., 
%Y.-C. Jang and W. Lee,
\pos{PoS(LATTICE2014)XXX}
[{\tt arXiv:XXXX.XXXX [hep-lat]}].
%
\bibitem{JWL}
J.~A.~Bailey {\it et al}., 
%[Fermilab Lattice and MILC Collaborations], 
\emph{Phys. Rev.} {\bf D89} (2014) 114504
[{\tt arXiv:1403.0635 [hep-lat]}]
%
\bibitem{GS} 
P.~Gambino and C.~Schwanda,
\emph{Phys. Rev.} {\bf D89} (2014) 014022
[{\tt arXiv:1307.4551 [hep-ph]}].
%
\bibitem{OK}
M. B. Oktay and A. S. Kronfeld,
\emph{Phys. Rev.} {\bf D78} (2008) 014504
[{\tt arXiv:0803.0523 [hep-lat]}].
%
\bibitem{Collins}
S.~Collins {\it et al}., 
\emph{Nucl. Phys. B Proc. Suppl.} {\bf 47} (1996) 455
[{\tt hep-lat/9512026}].
%
\bibitem{Kronfeld}
A.~S.~Kronfeld, 
\emph{Nucl. Phys. B Proc. Suppl.} {\bf 53} (1997) 401
[{\tt hep-lat/9608139}].
%
\bibitem{EKM}
A. X. El-Khadra, A. S. Kronfeld, and P. B. Mackenzie,
\emph{Phys. Rev.} {\bf D55} (1997) 3933 
[{\tt hep-lat/9604004}].
%
\bibitem{MBO:LAT2010}
C. DeTar, A. S. Kronfeld, and M. B. Oktay, 
\pos{PoS(LATTICE2010)234}
[{\tt arXiv:1011.5189 [hep-lat]}].
%
\bibitem{Bazavov:RevModPhys.82.1349}
A.~Bazavov {\it et al}.,
\emph{Rev. Mod. Phys.} {\bf 82} (2010) 1349
[{\tt arXiv:0903.3598 [hep-lat]}]
%
\bibitem{Wingate}
M.~Wingate {\it et al}., 
\emph{Phys. Rev.} {\bf D67} (2003) 054505
[{\tt hep-lat/0211014}].
%
\bibitem{Bernard}
C.~Bernard {\it et al}., 
\emph{Phys. Rev.} {\bf D83} (2011) 034503
[{\tt arXiv:1003.1937 [hep-lat]}].
%
\bibitem{JAB:LAT2014}
J.~A.~Bailey {\it et al}.,
%Y.-C. Jang, W. Lee, and J. Leem, 
\pos{PoS(LATTICE2014)XXX}
[{\tt arXiv:xxxxxx [hep-lat]}].
%
\bibitem{JANG:LAT2013}
Y.-C Jang {\it et al}.,
\pos{PoS(LATTICE2013)030}
[{\tt arXiv:1311.5029 [hep-lat]}].

\end{thebibliography}


==> tables/meson-mass.tex <==
\begin{table}[t]
%\footnotesize
\tabcolsep 3pt
\centering
\renewcommand{\arraystretch}{1.2}
%\resizebox{.8\textwidth}{!}{
\begin{tabular}{ c | c c c c}
  \hline \hline
  $\kappa$ & 0.038 & 0.039 & 0.040 & 0.041 \\
  \hline
  $a M(B_{s})$    & 3.99 & 3.65 & 3.32 & 3.01 \\
  $a M(\eta_{b})$ & 6.75 & 6.17 & 5.61 & 5.06 \\
  \hline\hline
\end{tabular}
%}
\caption{Meson masses (Pseudo-scalar)}
 \label{tbl:meson-mass}
\end{table}

